Efficient Image Denoising Using Global and Local Circulant Representation

The advancement of imaging devices and countless image data generated everyday impose an increasingly high demand on efficient and effective image denoising. In this paper, we present a computationally simple denoising algorithm, termed Haar-tSVD, aiming to explore the nonlocal self-similarity prior and leverage the connection between principal component analysis (PCA) and the Haar transform under circulant representation. We show that global and local patch correlations can be effectively captured through a unified tensor-singular value decomposition (t-SVD) projection with the Haar transform. This results in a one-step, highly parallelizable filtering method that eliminates the need for learning local bases to represent image patches, striking a balance between denoising speed and performance. Furthermore, we introduce an adaptive noise estimation scheme based on a CNN estimator and eigenvalue analysis to enhance the robustness and adaptability of the proposed method. Experiments on different real-world denoising tasks validate the efficiency and effectiveness of Haar-tSVD for noise removal and detail preservation. Datasets, code and results are publicly available at https://github.com/ZhaomingKong/Haar-tSVD.

==> Fig_HUAWEI-Mate40Pro_IPHONE13_compare.tex <==
\begin{figure}[htbp]
\graphicspath{{Figs_supplementary_TPAMI/Fig_images_Supp_proposed_dataset/Combined/}}
\centering
\subfigure[HUAWEI Mate40Pro]{
\label{Fig4}
\includegraphics[width=1.28in]{Huawei_Mate40Pro_IMG15_6_noisy_combined}}
\subfigure[IPHONE 13]{
\label{Fig4}
\includegraphics[width=1.28in]{IPHONE13_IMG39_9_noisy_combined}}

\caption{Images captured by two popular smartphones in dark environment.}
\label{Fig_HUAWEI-Mate40Pro_IPHONE13_compare}
\end{figure}


==> Fig_HUAWEI-Mate40Pro_dark_environment_demo.tex <==
\begin{figure}[htbp]
\graphicspath{{Figs_supplementary_TPAMI/Fig_images_Supp_proposed_dataset/}}
\centering
\subfigure[Trees]{
\label{Fig4}
\includegraphics[width=1.08in]{HuaweiMate40Pro_demo1}}
\subfigure[Streetlight]{
\label{Fig4}
\includegraphics[width=1.08in]{HuaweiMate40Pro_demo2}}
\subfigure[Grass]{
\label{Fig4}
\includegraphics[width=1.08in]{HuaweiMate40Pro_demo3}}

\caption{Images captured by HUAWEI Mate40Pro in dark environments.}
\label{Fig_HUAWEI-Mate40Pro_dark_environment_demo}
\end{figure}


==> Fig_HUAWEI-Mate40Pro_different_environment_demo.tex <==
%\begin{figure}[htbp]
%\graphicspath{{C:/Users/KZM11/Desktop/Fig_images_Supp_proposed_dataset/Combined/}}
%\centering
%\subfigure[Morning]{
%\label{Fig4}
%\includegraphics[width=1.08in]{Demo_HUAWEI_Mate40Pro_sufficient-light_combined_marked}}
%\subfigure[Afternoon]{
%\label{Fig4}
%\includegraphics[width=1.08in]{Demo_HUAWEI_Mate40Pro_low-light_combined}}
%\subfigure[Midnight]{
%\label{Fig4}
%\includegraphics[width=1.08in]{Demo_HUAWEI_Mate40Pro_dark_combined}}
%
%\caption{Images of HUAWEI Mate40Pro under different lighting conditions.}
%\label{Fig_HUAWEI-Mate40Pro_different_environment_demo}
%\end{figure}


\begin{figure}[htbp]
\graphicspath{{Figs_supplementary_TPAMI/Fig_images_Supp_proposed_dataset/Combined/}}
\centering
\subfigure[Morning]{
\label{Fig4}
\includegraphics[width=1.08in]{Demo_IPHONE13_sufficient-light_combined_marked}}
\subfigure[Afternoon]{
\label{Fig4}
\includegraphics[width=1.08in]{Demo_IPHONE13_low-light_combined}}
\subfigure[Midnight]{
\label{Fig4}
\includegraphics[width=1.08in]{Demo_IPHONE13_dark_combined}}

\caption{Images captured by IPHONE 13 under different lighting conditions.}
\label{Fig_HUAWEI-Mate40Pro_different_environment_demo}
\end{figure}


==> Fig_HUAWEI-Mate40Pro_noise_pattern_compare.tex <==
\begin{figure}[htbp]
\graphicspath{{Figs_supplementary_TPAMI/Fig_images_Supp_proposed_dataset/Combined/}}
\centering
\subfigure[Cups]{
\label{Fig4}
\includegraphics[width=0.81in]{Huawei_Mate40Pro_IMG4_2_noisy_combined}}
\subfigure[Streetlight]{
\label{Fig4}
\includegraphics[width=0.81in]{Huawei_Mate40Pro_IMG13_3_noisy_combined}}
\subfigure[Building A]{
\label{Fig4}
\includegraphics[width=0.81in]{Huawei_Mate40Pro_IMG30_6_noisy_combined}}
\subfigure[Building B]{
\label{Fig4}
\includegraphics[width=0.81in]{Huawei_Mate40Pro_IMG28_1_noisy_combined}}

\caption{Images captured by HUAWEI Mate40Pro of different scenes.}
\label{Fig_HUAWEI-Mate40Pro_noise_pattern_compare}
\end{figure}


==> Fig_Kong_dataset.tex <==
\begin{figure}[htbp]
\graphicspath{{Figs/Fig_dataset_illus/}}
\centering
\subfigure[The proposed IOCI dataset]{
\label{Fig4}
\includegraphics[width=3.38in]{Kong-Image}}
\subfigure[The proposed IOCV dataset]{
\label{Fig4}
\includegraphics[width=3.38in]{Kong-Video}}


\caption{Illustration of the proposed IOCI and IOCV dataset.}
\label{Fig_Kong_dataset}
\end{figure}


==> Fig_NSS.tex <==
\begin{figure}[htbp]
\graphicspath{{Figs/Frameworks/}}
\centering
\subfigure[Image data]{
\label{Fig4}
\includegraphics[width=0.78in]{Color_image}}
\subfigure[Video data]{
\label{Fig4}
\includegraphics[width=0.78in]{Color_video}}
\subfigure[MRI data]{
\label{Fig4}
\includegraphics[width=0.78in]{MRI}}
\subfigure[MSI data]{
\label{Fig4}
\includegraphics[width=0.78in]{MSI}}


\caption{The nonlocal self-similarity (NLSS) prior and patch representation of different imaging sensors, techniques and applications.}
\label{Fig_NSS}
\end{figure}


==> Fig_Video_slider.tex <==
\begin{figure}[htbp]
\graphicspath{{Figs/Fig_dataset_illus/}}
\vspace{-6.8pt}
\centering
\includegraphics[width=3.58in]{Video_slider}
\caption{The procedure of producing mean sequences with a motorized slider. The camera is fixed to a rotatable tripod ball-head placed on
top of the slider.}

\label{Fig_Video_slider}
\end{figure}


==> Fig_choose_N_noisy_for_mean_image.tex <==
\begin{figure}[htbp]
\graphicspath{{Figs_supplementary_TPAMI/Figs_Supp_Experiments_Image_dataset/}}
\centering
\subfigure[Relative error]{
\label{Fig4}
\includegraphics[width=1.666in]{Fig_Compare_mean_GT_img_relative_error}}
\subfigure[SSIM]{
\label{Fig4}
\includegraphics[width=1.666in]{Fig_Compare_mean_GT_img_SSIM}}

\caption{Relative error and SSIM of different mean images compared to the ground-truth. The camera device is IPHONE 13.}
\label{Fig_choose_N_noisy_for_mean_image}
\end{figure}


==> Fig_compare_Haar_A_Haar_SIDD.tex <==
\begin{figure}[htbp]
\vspace{-6.8pt}
\graphicspath{{Figs/Selected_color_images/SIDD/Selected_SIDD/Combined/Case5/}}
\centering
\subfigure[Noisy]{
\label{Fig4}
\includegraphics[width=0.8116in]{noisy_img31_13_combined_marked}}\hfill
\subfigure[CBM3D]{
\label{Fig4}
\includegraphics[width=0.8116in]{CBM3D2_img_31_13_sigma_85_combined_marked_new}}\hfill
\subfigure[Haar-tSVD]{
\label{Fig4}
\includegraphics[width=0.8116in]{CMStSVD_img_31_13_sigma_85_combined_marked}}\hfill
\subfigure[A-Haar-tSVD]{
\label{Fig4}
\includegraphics[width=0.8116in]{GCP-Haar31_13_sigma_40_combined_marked}}
\vspace{-3.8pt}
\caption{Denoising comparison on the Cuprite data [ref].}
\label{Fig_compare_Haar_A_Haar_SIDD}
\end{figure}


==> Fig_compare_OASIS.tex <==
\begin{figure}[htbp]
\vspace{-9.8pt}
\graphicspath{{Figs/Selected_color_images/MRI_OASIS/}}
\centering
\subfigure[MRI\_0092]{
\label{Fig4}
\includegraphics[width=3.2116in]{MRI_0092_combined}} \hfill
\vspace{-1.8pt}
\subfigure[MRI\_0112]{
\label{Fig4}
\includegraphics[width=3.2116in]{MRI_0112_combined}}\hfill
\vspace{-3.98pt}
\caption{Denoising results comparison on the OASIS dataset. The first and the second rows denote the denoised results and difference images, respectively.}
\label{Fig_compare_OASIS}
\end{figure}


==> Fig_compare_with_IOCI_FUJI.tex <==
\begin{figure}[htbp]
\vspace{-9.8pt}
\graphicspath{{Figs/Selected_color_images/IOCI/Case5/Combined/}}
\centering
\subfigure[Clean]{
\label{Fig4}
\includegraphics[width=0.8116in]{Fuji_X100T_IMG10_2_clean_combined_marked}} \hfill
\subfigure[Noisy]{
\label{Fig4}
\includegraphics[width=0.8116in]{Fuji_X100T_IMG10_2_noisy_combined_marked}}\hfill
\subfigure[Condformer]{
\label{Fig4}
\includegraphics[width=0.8116in]{Fuji_X100T_IMG10_2_noisy_Condformer_combined_marked}}\hfill
\subfigure[DeepSN]{
\label{Fig4}
\includegraphics[width=0.8116in]{Fuji_X100T_IMG10_2_noisy_DeepSN_combined_marked}}\hfill
\vspace{-6.8pt}
\subfigure[DIDN]{
\label{Fig4}
\includegraphics[width=0.8116in]{Fuji_X100T_IMG10_2_noisy_DIDN_combined_marked}}\hfill
\subfigure[NAFNet]{
\label{Fig4}
\includegraphics[width=0.8116in]{Fuji_X100T_IMG10_2_noisy_NAFNet_combined_marked}}\hfill
\subfigure[Restormer]{
\label{Fig4}
\includegraphics[width=0.8116in]{Fuji_X100T_IMG10_2_noisy_Restormer_combined_marked}}\hfill
\subfigure[A-Haar-tSVD]{
\label{Fig4}
\includegraphics[width=0.8116in]{Haar-tSVD_hand_tune_10_2_combined_marked}}
\vspace{-2.8pt}
\caption{Denoising results of compared methods on the IOCI datset.}
\label{Fig_compare_with_IOCI_FUJI}
\end{figure}


==> Fig_discussion_visual_enhancement.tex <==
\begin{figure}[htbp]
\graphicspath{{Figs/Fig_discussion/}}
\centering
\subfigure[Noisy (RENOIR)]{
\label{Fig4}
\includegraphics[width=1.08in]{Noisy_demo_combine_marked}}
\subfigure[CMSt-SVD]{
\label{Fig4}
\includegraphics[width=1.08in]{denoised_demo_combine}}
\subfigure[CMSt-SVD\_R]{
\label{Fig4}
\includegraphics[width=1.08in]{resized_demo_combine}}

\subfigure[Noisy (DND)]{
\label{Fig4}
\includegraphics[width=1.08in]{Noisy_demo2_combine_marked}}
\subfigure[CMSt-SVD]{
\label{Fig4}
\includegraphics[width=1.08in]{denoised_demo2_combine}}
\subfigure[CMSt-SVD\_R]{
\label{Fig4}
\includegraphics[width=1.08in]{resized_demo2_combine}}


\caption{Visual evaluation of CMSt-SVD with and without the image resizing strategy on RENOIR (first row) and DND (second row) datasets.}
\label{Fig_discussion_visual_enhancement}
\end{figure}


==> Fig_fastMRI.tex <==
\begin{figure*}[htbp]
\graphicspath{{Figs/combined_fastMRI/}}
\centering
\subfigure[Clean]{
\label{Fig4}
\includegraphics[width=0.81in]{Clean_img_9_slice_26_combined_marked}}
\subfigure[Noisy]{
\label{Fig4}
\includegraphics[width=0.81in]{Noisy_img_9_slice_26_Sigma3_combined}}
\subfigure[4DHOSVD]{
\label{Fig4}
\includegraphics[width=0.81in]{4DHOSVD1_img_9_slice_26_Sigma3_combined}}
\subfigure[AONLM]{
\label{Fig4}
\includegraphics[width=0.81in]{AONLM_img_9_slice_26_Sigma3_combined}}
\subfigure[BM4D2]{
\label{Fig4}
\includegraphics[width=0.81in]{BM4D2_img_9_slice_26_Sigma3_combined}}
\subfigure[ILR-HOSVD]{
\label{Fig4}
\includegraphics[width=0.81in]{ILRHOSVD_img_9_slice_26_Sigma3_combined}}
\subfigure[MSt-SVD]{
\label{Fig4}
\includegraphics[width=0.81in]{MStSVD_img_9_slice_26_Sigma3_combined}}
\subfigure[ODCT]{
\label{Fig4}
\includegraphics[width=0.81in]{ODCT_img_9_slice_26_Sigma3_combined}}

\subfigure[Clean]{
\label{Fig4}
\includegraphics[width=0.81in]{Clean_img_9_slice_26_combined_marked}}
\subfigure[Noisy]{
\label{Fig4}
\includegraphics[width=0.81in]{Noisy_img_9_slice_26_Sigma11_combined}}
\subfigure[4DHOSVD]{
\label{Fig4}
\includegraphics[width=0.81in]{4DHOSVD1_img_9_slice_26_Sigma11_combined}}
\subfigure[AONLM]{
\label{Fig4}
\includegraphics[width=0.81in]{AONLM_img_9_slice_26_Sigma11_combined}}
\subfigure[BM4D2]{
\label{Fig4}
\includegraphics[width=0.81in]{BM4D2_img_9_slice_26_Sigma11_combined}}
\subfigure[ILR-HOSVD]{
\label{Fig4}
\includegraphics[width=0.81in]{ILRHOSVD_img_9_slice_26_Sigma11_combined}}
\subfigure[MSt-SVD]{
\label{Fig4}
\includegraphics[width=0.81in]{MStSVD_img_9_slice_26_Sigma11_combined}}
\subfigure[ODCT]{
\label{Fig4}
\includegraphics[width=0.81in]{ODCT_img_9_slice_26_Sigma11_combined}}


\subfigure[Clean]{
\label{Fig4}
\includegraphics[width=0.81in]{Clean_img_9_slice_26_combined_marked}}
\subfigure[Noisy]{
\label{Fig4}
\includegraphics[width=0.81in]{Noisy_img_9_slice_26_Sigma19_combined}}
\subfigure[4DHOSVD]{
\label{Fig4}
\includegraphics[width=0.81in]{4DHOSVD1_img_9_slice_26_Sigma19_combined}}
\subfigure[AONLM]{
\label{Fig4}
\includegraphics[width=0.81in]{AONLM_img_9_slice_26_Sigma19_combined}}
\subfigure[BM4D2]{
\label{Fig4}
\includegraphics[width=0.81in]{BM4D2_img_9_slice_26_Sigma19_combined}}
\subfigure[ILR-HOSVD]{
\label{Fig4}
\includegraphics[width=0.81in]{ILRHOSVD_img_9_slice_26_Sigma19_combined}}
\subfigure[MSt-SVD]{
\label{Fig4}
\includegraphics[width=0.81in]{MStSVD_img_9_slice_26_Sigma19_combined}}
\subfigure[ODCT]{
\label{Fig4}
\includegraphics[width=0.81in]{ODCT_img_9_slice_26_Sigma19_combined}}


\caption{Visual evaluation of the fastMRI dataset at different Rician noise levels. From the first row to the third row: $\sigma$ = 3\%, $\sigma$ = 11\% and $\sigma$ = 19\%.}
\label{Fig_fastMRI}
\end{figure*}


==> Table_Color_Image_time.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
\scriptsize
  \centering
  \caption{Add caption}
  \scalebox{0.8}{
    \begin{tabular}{cccccccccc}
    \toprule
    NLH-CC & CBM3D & MSt-SVD & Haar-tSVD & A-Haar-tSVD & AP-BSN & Ne2Ne & S2S   & FFDNet & Restormer \\
    \midrule
    40.32 & 2.94  & 4.95  & 2.68  & 3.12  & 3.56  & 2.48  & >1000 & 0.02  & 0.77 \\
    \bottomrule
    \end{tabular}}%
  \label{tab:addlabel}%
\end{table}%


==> Table_dataset_info.tex <==
% Table generated by Excel2LaTeX from sheet 'TMM'
\begin{table}[htbp]
\scriptsize
  \centering
  \caption{Popular image/video denoising datasets. `GT': ground-truth, `A': Available, `N/A': Not-Available, `F': number of frames.} 
  \scalebox{0.88}{
    \begin{tabular}{cccccc}
    \toprule
    Applications & Name  & Experiments & GT    & Image size & \# Images \\
    \midrule
    \multicolumn{1}{c}{\multirow{8}[16]{*}{Image}} & Kodak \cite{Kodak} & Synthetic & A     & 512 x 512 x 3 & 24 \\
\cmidrule{2-6}          & RENOIR \cite{anaya2018renoir} & Real-world & A     & 3684 x 2760 x 3 & 120 \\
\cmidrule{2-6}          & Nam \cite{nam2016holistic} & Real-world & A     & 512 x 512 x 3 & 15 \\
\cmidrule{2-6}          & PolyU \cite{xu2018real} & Real-world & A     & 512 x 512 x 3 & 100 \\
\cmidrule{2-6}          & DnD \cite{plotz2017benchmarking} & Real-world & N/A   & 512 x 512 x 3 & 1000 \\
\cmidrule{2-6}          & SIDD \cite{abdelhamed2018high} & Real-world & N/A   & 256 x 256 x 3 & 1280 \\
\cmidrule{2-6}          & High-ISO \cite{yue2019high} & Real-world & A     & 512 x 512 x 3 & 100 \\
\cmidrule{2-6}          & IOCI \cite{kong2023comparison} & Real-world & A     & 1024 x 1024 x 3 & 848 \\
    \midrule
    \multirow{5}[3]{*}{Video} & Set8 \cite{Set8} & Synthetic & A     & 960 x 540 x 3 x F & 8 \\
\cmidrule{2-6}          & DAVIS \cite{Perazzi2016} & Synthetic & A     & 854 x 480 x 3 x F & 30 \\
\cmidrule{2-6}          & CRVD \cite{yue2020supervised} & Real-world & A     & 1920 x 1080 x 3 x F & 61 \\
%\cmidrule{2-6}          & PVDD \cite{xu2022pvdd} & Real-world & A & Unknown & 200 \\
\cmidrule{2-6}          & IOCV \cite{kong2023comparison} & Real-world & A     & 512 x 512 x 3 x F & 39 \\
    \bottomrule
    \end{tabular}}%
  \label{Table_dataset_info}%
\end{table}%

